Classification-based Quality Estimation: Small and Efficient Models for Real-world Applications

Sentence-level Quality estimation (QE) of machine translation is traditionally formulated as a regression task, and the performance of QE models is typically measured by Pearson correlation with human labels. Recent QE models have achieved previously-unseen levels of correlation with human judgments, but they rely on large multilingual contextualized language models that are computationally expensive and make them infeasible for real-world applications. In this work, we evaluate several model compression techniques for QE and find that, despite their popularity in other NLP tasks, they lead to poor performance in this regression setting. We observe that a full model parameterization is required to achieve SoTA results in a regression task. However, we argue that the level of expressiveness of a model in a continuous range is unnecessary given the downstream applications of QE, and show that reframing QE as a classification problem and evaluating QE models using classification metrics would better reflect their actual performance in real-world applications.

==> results/binary_blog.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{6}{*}{blog}&\multirow{3}{*}{base}&\multirow{2}{*}{REG}&\multirow{1}{*}{PC}&BL&0.45&0.52&0.54&0.57&0.46&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{1}{*}{F1}&BL&\textbf{0.60}&0.61&0.53&\textbf{0.62}&0.59&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{1}{*}{CLS}&\multirow{1}{*}{F1}&BL&0.58&\textbf{0.63}&\textbf{0.64}&\textbf{0.62}&\textbf{0.61}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{3}{*}{large}&\multirow{2}{*}{REG}&\multirow{1}{*}{PC}&BL&0.47&0.51&0.51&0.51&0.55&0.58&0.58&0.58&0.56\\
\cmidrule{5-14}
&&&\multirow{1}{*}{F1}&BL&\textbf{0.60}&0.61&0.62&0.61&0.60&0.62&0.62&0.63&0.59\\
\cmidrule{3-14}
&&\multirow{1}{*}{CLS}&\multirow{1}{*}{F1}&BL&0.59&\textbf{0.63}&\textbf{0.64}&\textbf{0.63}&\textbf{0.64}&\textbf{0.65}&\textbf{0.65}&\textbf{0.65}&\textbf{0.65}\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Blog (Binary F1)
}
\end{table*}

==> results/binary_high.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{en-de}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.22&0.32&0.33&0.37&0.46&-&-&-&-\\
&&&&ML&0.11&0.33&0.29&0.37&0.37&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&-&-&-&-\\
&&&&ML&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&-&-&-&-\\
&&&&ML&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.29&0.33&0.36&0.37&0.47&0.50&0.52&0.51&0.50\\
&&&&ML&0.21&0.33&0.33&0.40&0.46&0.47&0.47&0.48&0.49\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}\\
&&&&ML&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}\\
&&&&ML&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}&\textbf{0.99}\\
\bottomrule
\multirow{12}{*}{en-zh}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.27&0.32&0.32&0.40&0.44&-&-&-&-\\
&&&&ML&0.18&0.26&0.29&0.39&0.40&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&-&-&-&-\\
&&&&ML&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&-&-&-&-\\
&&&&ML&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.27&0.32&0.33&0.35&0.43&0.48&0.50&0.51&0.51\\
&&&&ML&0.20&0.24&0.30&0.32&0.44&0.45&0.46&0.45&0.47\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}\\
&&&&ML&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}\\
&&&&ML&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}\\
\bottomrule
\multirow{12}{*}{ru-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.63&0.64&0.66&0.69&0.73&-&-&-&-\\
&&&&ML&0.55&0.64&0.68&0.72&0.73&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.89}&\textbf{0.88}&\textbf{0.89}&\textbf{0.89}&\textbf{0.90}&-&-&-&-\\
&&&&ML&0.86&\textbf{0.88}&\textbf{0.89}&\textbf{0.89}&\textbf{0.89}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.85&\textbf{0.88}&0.88&\textbf{0.89}&\textbf{0.90}&-&-&-&-\\
&&&&ML&0.85&\textbf{0.88}&0.88&\textbf{0.89}&\textbf{0.90}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.62&0.67&0.67&0.68&0.71&0.74&0.78&0.79&0.80\\
&&&&ML&0.57&0.66&0.67&0.68&0.75&0.76&0.79&0.80&0.79\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.88}&\textbf{0.89}&\textbf{0.89}&\textbf{0.89}&\textbf{0.90}&\textbf{0.90}&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}\\
&&&&ML&0.87&0.88&\textbf{0.89}&0.88&\textbf{0.90}&0.89&\textbf{0.91}&\textbf{0.91}&\textbf{0.91}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.88}&0.88&\textbf{0.89}&\textbf{0.89}&0.89&0.89&0.90&\textbf{0.91}&\textbf{0.91}\\
&&&&ML&0.85&0.88&\textbf{0.89}&\textbf{0.89}&0.89&\textbf{0.90}&0.90&\textbf{0.91}&\textbf{0.91}\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
High resource LDs (Binary F1)
}
\end{table*}

==> results/binary_low.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{si-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.43&0.47&0.52&0.56&0.59&-&-&-&-\\
&&&&ML&0.35&0.44&0.52&0.59&0.59&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.61&\textbf{0.70}&\textbf{0.73}&\textbf{0.73}&\textbf{0.73}&-&-&-&-\\
&&&&ML&0.60&0.64&0.71&0.72&0.72&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.69}&0.69&0.72&\textbf{0.73}&\textbf{0.73}&-&-&-&-\\
&&&&ML&0.68&0.68&0.68&0.69&0.72&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.44&0.47&0.48&0.50&0.57&0.60&0.61&0.64&0.65\\
&&&&ML&0.38&0.47&0.50&0.52&0.60&0.62&0.65&0.66&0.65\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.66&\textbf{0.72}&0.71&0.71&0.72&0.73&\textbf{0.74}&\textbf{0.74}&0.73\\
&&&&ML&0.67&0.71&\textbf{0.73}&\textbf{0.72}&\textbf{0.73}&\textbf{0.74}&0.73&0.73&0.71\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.69}&0.70&0.71&0.71&0.72&0.73&0.73&\textbf{0.74}&\textbf{0.74}\\
&&&&ML&0.66&0.68&0.69&0.70&0.72&0.73&0.73&0.73&0.71\\
\bottomrule
\multirow{12}{*}{ne-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.52&0.55&0.59&0.70&0.70&-&-&-&-\\
&&&&ML&0.41&0.50&0.59&0.68&0.69&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.41}&\textbf{0.47}&\textbf{0.51}&0.54&0.57&-&-&-&-\\
&&&&ML&0.09&0.36&\textbf{0.51}&\textbf{0.57}&\textbf{0.57}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.06&0.25&0.06&0.44&0.55&-&-&-&-\\
&&&&ML&0.15&0.34&0.29&0.55&\textbf{0.58}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.52&0.57&0.57&0.59&0.72&0.74&0.75&0.77&0.78\\
&&&&ML&0.45&0.53&0.56&0.57&0.70&0.74&0.77&0.78&0.77\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.40}&\textbf{0.52}&\textbf{0.52}&\textbf{0.51}&0.56&0.60&0.61&0.62&0.64\\
&&&&ML&0.26&0.45&0.49&0.49&\textbf{0.60}&\textbf{0.62}&\textbf{0.65}&\textbf{0.66}&\textbf{0.65}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.00&0.47&0.49&\textbf{0.51}&0.58&0.61&0.62&0.64&0.63\\
&&&&ML&0.02&0.33&0.39&0.50&\textbf{0.60}&\textbf{0.62}&\textbf{0.65}&0.65&\textbf{0.65}\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Low resource LDs (Binary F1)
}
\end{table*}

==> results/binary_mid.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{ro-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.65&0.71&0.74&0.81&0.84&-&-&-&-\\
&&&&ML&0.46&0.64&0.71&0.82&0.83&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.88}&\textbf{0.88}&0.89&0.90&\textbf{0.91}&-&-&-&-\\
&&&&ML&0.87&\textbf{0.88}&\textbf{0.90}&\textbf{0.91}&\textbf{0.91}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.86&\textbf{0.88}&0.88&0.90&0.90&-&-&-&-\\
&&&&ML&0.86&0.87&0.88&\textbf{0.91}&0.90&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.62&0.69&0.71&0.72&0.85&0.85&0.87&0.88&0.88\\
&&&&ML&0.51&0.67&0.69&0.67&0.85&0.85&0.87&0.88&0.87\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.88}&\textbf{0.89}&\textbf{0.90}&\textbf{0.90}&\textbf{0.91}&\textbf{0.92}&\textbf{0.92}&\textbf{0.92}&\textbf{0.92}\\
&&&&ML&\textbf{0.88}&\textbf{0.89}&0.89&0.89&\textbf{0.91}&\textbf{0.92}&\textbf{0.92}&\textbf{0.92}&\textbf{0.92}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.86&\textbf{0.89}&0.89&0.89&\textbf{0.91}&0.91&\textbf{0.92}&\textbf{0.92}&0.91\\
&&&&ML&0.86&0.88&0.89&0.89&\textbf{0.91}&0.91&\textbf{0.92}&\textbf{0.92}&\textbf{0.92}\\
\bottomrule
\multirow{12}{*}{et-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.48&0.51&0.58&0.64&0.67&-&-&-&-\\
&&&&ML&0.35&0.52&0.59&0.68&0.68&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.73}&\textbf{0.76}&\textbf{0.77}&0.77&\textbf{0.78}&-&-&-&-\\
&&&&ML&0.72&\textbf{0.76}&0.76&0.77&0.77&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.72&0.74&0.76&\textbf{0.78}&\textbf{0.78}&-&-&-&-\\
&&&&ML&0.72&0.75&0.75&0.77&0.77&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.47&0.55&0.56&0.61&0.69&0.72&0.76&0.78&0.78\\
&&&&ML&0.38&0.54&0.56&0.59&0.72&0.75&0.79&0.79&0.79\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.74}&\textbf{0.76}&\textbf{0.76}&\textbf{0.76}&0.77&0.77&0.78&0.80&0.81\\
&&&&ML&0.72&0.75&0.75&0.75&0.77&\textbf{0.78}&\textbf{0.81}&0.81&0.80\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.72&\textbf{0.76}&\textbf{0.76}&\textbf{0.76}&\textbf{0.78}&\textbf{0.78}&0.79&\textbf{0.82}&\textbf{0.83}\\
&&&&ML&0.72&0.75&0.75&\textbf{0.76}&\textbf{0.78}&\textbf{0.78}&0.80&0.81&0.81\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Mid resource LDs (Binary F1)
}
\end{table*}

==> results/macro_blog.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{6}{*}{blog}&\multirow{3}{*}{base}&\multirow{2}{*}{REG}&\multirow{1}{*}{PC}&BL&0.45&0.52&0.54&0.57&0.46&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{1}{*}{F1}&BL&0.35&0.46&0.46&0.49&0.35&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{1}{*}{CLS}&\multirow{1}{*}{F1}&BL&\textbf{0.47}&\textbf{0.55}&\textbf{0.56}&\textbf{0.57}&\textbf{0.53}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{3}{*}{large}&\multirow{2}{*}{REG}&\multirow{1}{*}{PC}&BL&0.47&0.51&0.51&0.51&0.55&0.58&0.58&0.58&0.56\\
\cmidrule{5-14}
&&&\multirow{1}{*}{F1}&BL&0.36&0.43&0.43&0.43&0.47&0.50&0.50&0.48&0.47\\
\cmidrule{3-14}
&&\multirow{1}{*}{CLS}&\multirow{1}{*}{F1}&BL&\textbf{0.52}&\textbf{0.55}&\textbf{0.55}&\textbf{0.54}&\textbf{0.57}&\textbf{0.59}&\textbf{0.60}&\textbf{0.60}&\textbf{0.59}\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Blog (Macro F1)
}
\end{table*}

==> results/macro_high.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{en-de}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.22&0.32&0.33&0.37&0.46&-&-&-&-\\
&&&&ML&0.11&0.33&0.29&0.37&0.27&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.13&0.17&0.16&0.16&0.17&-&-&-&-\\
&&&&ML&0.15&0.09&0.16&\textbf{0.29}&0.17&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.16}&\textbf{0.23}&0.21&0.21&\textbf{0.23}&-&-&-&-\\
&&&&ML&0.15&0.12&\textbf{0.25}&0.23&0.13&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.29&0.33&0.36&0.37&0.47&0.50&0.52&0.51&0.50\\
&&&&ML&0.21&0.33&0.33&0.40&0.46&0.47&0.47&0.48&0.45\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.11&0.17&0.14&0.15&0.15&0.17&0.17&0.17&0.12\\
&&&&ML&0.13&0.17&0.16&0.17&0.18&0.16&0.18&0.20&0.17\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.16}&\textbf{0.23}&\textbf{0.21}&\textbf{0.21}&\textbf{0.24}&\textbf{0.24}&0.22&\textbf{0.25}&\textbf{0.23}\\
&&&&ML&0.14&0.13&0.12&0.13&0.18&0.21&\textbf{0.23}&0.22&0.19\\
\bottomrule
\multirow{12}{*}{en-zh}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.27&0.32&0.32&0.40&0.44&-&-&-&-\\
&&&&ML&0.18&0.26&0.29&0.39&0.27&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.18}&0.23&0.13&0.17&0.19&-&-&-&-\\
&&&&ML&\textbf{0.18}&\textbf{0.25}&0.18&0.20&0.19&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.17&0.14&\textbf{0.20}&\textbf{0.23}&\textbf{0.23}&-&-&-&-\\
&&&&ML&0.09&0.13&0.12&0.13&0.15&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.27&0.32&0.33&0.35&0.43&0.48&0.50&0.51&0.51\\
&&&&ML&0.20&0.24&0.30&0.32&0.44&0.45&0.46&0.45&0.45\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.19&0.19&0.18&0.17&0.16&0.16&0.19&0.19&0.22\\
&&&&ML&\textbf{0.23}&0.18&0.18&0.22&\textbf{0.20}&\textbf{0.20}&\textbf{0.23}&0.23&\textbf{0.26}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.11&\textbf{0.24}&\textbf{0.27}&\textbf{0.23}&\textbf{0.20}&0.19&0.22&\textbf{0.24}&\textbf{0.26}\\
&&&&ML&0.10&0.16&0.13&0.13&0.12&0.15&0.15&0.17&0.18\\
\bottomrule
\multirow{12}{*}{ru-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.63&0.64&0.66&0.69&0.73&-&-&-&-\\
&&&&ML&0.55&0.64&0.68&0.72&0.58&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.24}&0.24&0.26&0.30&0.31&-&-&-&-\\
&&&&ML&0.17&0.22&0.27&0.28&0.17&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.19&\textbf{0.32}&\textbf{0.34}&\textbf{0.36}&\textbf{0.34}&-&-&-&-\\
&&&&ML&0.16&0.27&0.29&0.29&0.24&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.62&0.67&0.67&0.68&0.71&0.74&0.78&0.79&0.80\\
&&&&ML&0.57&0.66&0.67&0.68&0.75&0.76&0.79&0.80&0.79\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.24&0.30&0.32&0.28&0.29&0.30&0.35&0.34&0.33\\
&&&&ML&0.20&0.25&0.26&0.24&0.29&0.27&0.31&0.34&0.34\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.32}&\textbf{0.33}&\textbf{0.34}&\textbf{0.35}&\textbf{0.36}&0.34&\textbf{0.36}&\textbf{0.39}&\textbf{0.40}\\
&&&&ML&0.16&0.28&0.29&0.30&0.32&\textbf{0.35}&0.35&0.35&0.33\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
High resource LDs (Macro F1)
}
\end{table*}

==> results/macro_low.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{si-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.43&0.47&0.52&0.56&0.59&-&-&-&-\\
&&&&ML&0.35&0.44&0.52&0.59&0.42&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.27}&\textbf{0.31}&\textbf{0.37}&\textbf{0.39}&\textbf{0.37}&-&-&-&-\\
&&&&ML&0.15&0.23&0.36&\textbf{0.39}&0.18&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.12&0.20&0.27&0.25&0.28&-&-&-&-\\
&&&&ML&0.10&0.23&0.26&0.31&0.09&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.44&0.47&0.48&0.50&0.57&0.60&0.61&0.64&0.65\\
&&&&ML&0.38&0.47&0.50&0.52&0.60&0.62&0.65&0.66&0.65\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.29}&\textbf{0.35}&\textbf{0.34}&\textbf{0.35}&0.36&0.40&0.40&0.45&\textbf{0.44}\\
&&&&ML&0.18&0.30&0.32&0.34&\textbf{0.39}&\textbf{0.41}&\textbf{0.43}&\textbf{0.46}&0.43\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.22&0.31&0.30&0.28&0.28&0.30&0.30&0.31&0.32\\
&&&&ML&0.10&0.22&0.23&0.25&0.28&0.27&0.30&0.28&0.32\\
\bottomrule
\multirow{12}{*}{ne-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.52&0.55&0.59&0.70&0.70&-&-&-&-\\
&&&&ML&0.41&0.50&0.59&0.68&0.49&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.22}&\textbf{0.24}&\textbf{0.27}&0.31&\textbf{0.35}&-&-&-&-\\
&&&&ML&0.12&0.23&\textbf{0.27}&\textbf{0.38}&0.21&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.17&0.22&0.24&0.31&0.33&-&-&-&-\\
&&&&ML&0.15&0.20&0.26&0.30&0.15&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.52&0.57&0.57&0.59&0.72&0.74&0.75&0.77&0.78\\
&&&&ML&0.45&0.53&0.56&0.57&0.70&0.74&0.77&0.78&0.77\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.25}&\textbf{0.31}&\textbf{0.30}&\textbf{0.28}&0.30&0.34&0.34&0.30&0.34\\
&&&&ML&0.17&0.21&0.23&0.23&0.32&\textbf{0.37}&\textbf{0.38}&\textbf{0.39}&\textbf{0.37}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.20&0.26&0.29&0.27&0.32&0.34&0.33&0.33&\textbf{0.37}\\
&&&&ML&0.15&0.21&0.21&0.25&\textbf{0.33}&\textbf{0.37}&0.36&0.37&0.28\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Low resource LDs (Macro F1)
}
\end{table*}

==> results/macro_mid.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{ro-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.65&0.71&0.74&0.81&0.84&-&-&-&-\\
&&&&ML&0.46&0.64&0.71&0.82&0.56&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.28}&\textbf{0.42}&\textbf{0.44}&\textbf{0.50}&0.50&-&-&-&-\\
&&&&ML&0.14&0.24&0.37&0.49&0.16&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.20&0.41&0.43&0.48&\textbf{0.51}&-&-&-&-\\
&&&&ML&0.13&0.32&0.35&0.39&0.25&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.62&0.69&0.71&0.72&0.85&0.85&0.87&0.88&0.88\\
&&&&ML&0.51&0.67&0.69&0.67&0.85&0.85&0.87&0.88&0.87\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.32&0.37&0.38&0.38&0.48&\textbf{0.53}&0.51&0.52&\textbf{0.55}\\
&&&&ML&0.17&0.33&0.31&0.28&0.47&0.46&0.50&\textbf{0.54}&0.50\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.36}&\textbf{0.43}&\textbf{0.44}&\textbf{0.45}&\textbf{0.49}&\textbf{0.53}&\textbf{0.52}&0.53&\textbf{0.55}\\
&&&&ML&0.14&0.26&0.31&0.33&0.39&0.45&0.46&0.47&0.47\\
\bottomrule
\multirow{12}{*}{et-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.48&0.51&0.58&0.64&0.67&-&-&-&-\\
&&&&ML&0.35&0.52&0.59&0.68&0.47&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.15}&0.19&0.19&0.21&\textbf{0.25}&-&-&-&-\\
&&&&ML&0.11&0.16&0.20&0.22&0.11&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.11&\textbf{0.24}&\textbf{0.26}&\textbf{0.25}&\textbf{0.25}&-&-&-&-\\
&&&&ML&0.10&0.20&0.17&0.16&0.20&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.47&0.55&0.56&0.61&0.69&0.72&0.76&0.78&0.78\\
&&&&ML&0.38&0.54&0.56&0.59&0.72&0.75&0.79&0.79&0.79\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.17&0.20&0.20&0.20&0.22&0.23&0.24&0.24&0.27\\
&&&&ML&0.12&0.17&0.17&0.16&0.22&0.22&\textbf{0.27}&0.27&0.26\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.23}&\textbf{0.25}&\textbf{0.25}&\textbf{0.25}&\textbf{0.24}&\textbf{0.26}&0.25&\textbf{0.32}&\textbf{0.33}\\
&&&&ML&0.10&0.19&0.19&0.17&0.20&0.20&0.21&0.23&0.26\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Mid resource LDs (Macro F1)
}
\end{table*}

==> results/micro_blog.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{6}{*}{blog}&\multirow{3}{*}{base}&\multirow{2}{*}{REG}&\multirow{1}{*}{PC}&BL&0.48&0.55&0.56&0.59&0.59&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{1}{*}{F1}&BL&\textbf{0.50}&\textbf{0.51}&\textbf{0.54}&\textbf{0.56}&\textbf{0.57}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{1}{*}{CLS}&\multirow{1}{*}{F1}&BL&0.43&0.48&0.52&0.54&\textbf{0.57}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{3}{*}{large}&\multirow{2}{*}{REG}&\multirow{1}{*}{PC}&BL&0.42&0.56&0.56&0.56&0.57&0.60&0.61&0.61&0.59\\
\cmidrule{5-14}
&&&\multirow{1}{*}{F1}&BL&\textbf{0.47}&\textbf{0.52}&0.52&\textbf{0.54}&0.52&0.57&0.58&0.55&0.55\\
\cmidrule{3-14}
&&\multirow{1}{*}{CLS}&\multirow{1}{*}{F1}&BL&0.42&0.49&\textbf{0.55}&0.48&\textbf{0.60}&\textbf{0.64}&\textbf{0.62}&\textbf{0.59}&\textbf{0.64}\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Blog (Micro F1)
}
\end{table*}

==> results/micro_high.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{en-de}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.19&0.15&0.32&0.38&0.46&-&-&-&-\\
&&&&ML&0.27&0.33&0.29&0.40&0.42&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.36&0.35&0.48&\textbf{0.51}&0.48&-&-&-&-\\
&&&&ML&0.38&0.37&0.46&0.47&\textbf{0.52}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.48}&\textbf{0.47}&\textbf{0.49}&0.50&0.51&-&-&-&-\\
&&&&ML&0.42&\textbf{0.47}&0.48&0.50&0.51&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.29&0.28&0.37&0.37&0.46&0.48&0.50&0.52&0.49\\
&&&&ML&0.26&0.34&0.31&0.39&0.46&0.48&0.46&0.46&0.48\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.40&0.45&0.45&0.46&0.48&0.50&0.47&0.51&0.42\\
&&&&ML&0.41&0.46&0.44&0.48&0.48&0.45&0.46&0.48&0.51\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.48}&\textbf{0.48}&\textbf{0.50}&\textbf{0.49}&\textbf{0.52}&\textbf{0.52}&0.51&0.51&0.52\\
&&&&ML&\textbf{0.48}&\textbf{0.48}&0.48&\textbf{0.49}&0.51&0.50&\textbf{0.53}&\textbf{0.52}&\textbf{0.54}\\
\bottomrule
\multirow{12}{*}{en-zh}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.29&0.32&0.33&0.40&0.44&-&-&-&-\\
&&&&ML&0.20&0.26&0.30&0.39&0.43&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.43}&\textbf{0.45}&0.30&0.35&0.36&-&-&-&-\\
&&&&ML&0.42&0.41&\textbf{0.39}&0.40&\textbf{0.39}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.28&0.28&0.31&\textbf{0.41}&\textbf{0.39}&-&-&-&-\\
&&&&ML&0.27&0.28&0.31&0.32&0.34&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.27&0.32&0.34&0.35&0.43&0.48&0.50&0.51&0.52\\
&&&&ML&0.21&0.23&0.29&0.34&0.44&0.44&0.45&0.45&0.48\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.42}&\textbf{0.43}&0.39&0.35&0.35&0.38&0.37&0.39&\textbf{0.44}\\
&&&&ML&0.40&0.40&\textbf{0.40}&0.39&0.42&0.40&0.42&0.44&0.43\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.28&\textbf{0.43}&\textbf{0.40}&\textbf{0.43}&\textbf{0.43}&\textbf{0.41}&\textbf{0.44}&\textbf{0.48}&0.42\\
&&&&ML&0.31&0.37&0.32&0.34&0.32&0.37&0.34&0.39&0.40\\
\bottomrule
\multirow{12}{*}{ru-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.64&0.64&0.66&0.69&0.73&-&-&-&-\\
&&&&ML&0.60&0.63&0.68&0.72&0.75&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.45&0.46&0.47&0.46&0.48&-&-&-&-\\
&&&&ML&0.42&0.45&0.45&0.47&0.44&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.47}&\textbf{0.49}&\textbf{0.49}&\textbf{0.50}&\textbf{0.50}&-&-&-&-\\
&&&&ML&0.39&0.44&0.45&0.42&0.47&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.62&0.65&0.67&0.68&0.71&0.74&0.77&0.78&0.81\\
&&&&ML&0.59&0.64&0.68&0.68&0.74&0.76&0.79&0.80&0.81\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.43&0.46&0.45&0.44&0.47&0.50&0.48&0.50&\textbf{0.53}\\
&&&&ML&0.41&0.42&0.43&0.41&0.46&0.48&0.48&0.49&0.50\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.47}&0.47&0.47&0.47&0.48&0.49&0.49&\textbf{0.52}&0.52\\
&&&&ML&\textbf{0.47}&\textbf{0.48}&\textbf{0.50}&\textbf{0.50}&\textbf{0.52}&\textbf{0.51}&\textbf{0.50}&\textbf{0.52}&\textbf{0.53}\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
High resource LDs (Micro F1)
}
\end{table*}

==> results/micro_low.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{si-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.43&0.44&0.51&0.56&0.60&-&-&-&-\\
&&&&ML&0.39&0.43&0.53&0.58&0.62&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&0.36&\textbf{0.36}&0.35&0.34&0.36&-&-&-&-\\
&&&&ML&\textbf{0.37}&0.35&\textbf{0.39}&\textbf{0.40}&\textbf{0.41}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.30&0.28&0.27&0.30&0.27&-&-&-&-\\
&&&&ML&0.23&0.17&0.26&0.27&0.27&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.44&0.48&0.48&0.50&0.57&0.60&0.61&0.63&0.65\\
&&&&ML&0.41&0.47&0.51&0.53&0.60&0.62&0.64&0.66&0.67\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.36}&\textbf{0.36}&\textbf{0.38}&\textbf{0.38}&0.33&0.36&0.37&0.40&0.42\\
&&&&ML&\textbf{0.36}&\textbf{0.36}&0.37&0.37&\textbf{0.40}&\textbf{0.41}&\textbf{0.41}&\textbf{0.43}&\textbf{0.44}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.24&0.30&0.33&0.34&0.32&0.34&0.31&0.32&0.32\\
&&&&ML&0.17&0.24&0.23&0.25&0.25&0.27&0.26&0.31&0.31\\
\bottomrule
\multirow{12}{*}{ne-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.52&0.55&0.60&0.69&0.70&-&-&-&-\\
&&&&ML&0.48&0.53&0.59&0.67&0.71&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.49}&\textbf{0.49}&0.45&0.41&0.47&-&-&-&-\\
&&&&ML&0.47&\textbf{0.49}&0.49&0.52&0.54&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.43&0.44&0.47&0.49&0.45&-&-&-&-\\
&&&&ML&0.41&0.39&\textbf{0.50}&\textbf{0.55}&\textbf{0.56}&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.52&0.54&0.57&0.59&0.72&0.73&0.75&0.77&0.77\\
&&&&ML&0.49&0.53&0.56&0.59&0.70&0.74&0.77&0.78&0.79\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.49}&0.45&0.44&0.43&0.44&0.49&0.45&0.50&0.45\\
&&&&ML&0.46&0.48&0.47&0.48&0.51&\textbf{0.53}&\textbf{0.56}&0.56&0.56\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.43&0.48&0.50&0.46&0.50&0.49&0.48&0.49&0.52\\
&&&&ML&0.44&\textbf{0.50}&\textbf{0.51}&\textbf{0.52}&\textbf{0.56}&\textbf{0.53}&0.55&\textbf{0.57}&\textbf{0.58}\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Low resource LDs (Micro F1)
}
\end{table*}

==> results/micro_mid.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
&&&&\multicolumn{9}{c}{\textbf{Layers}}\\
\cmidrule{4-14}
\textbf{LD}&\textbf{XLMR}&\textbf{OBJ}&\textbf{MTC}&\textbf{MDL}&\textbf{1}&\textbf{3}&\textbf{6}&\textbf{9}&\textbf{12}&\textbf{15}&\textbf{18}&\textbf{21}&\textbf{24}\\
\bottomrule
\multirow{12}{*}{ro-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.65&0.70&0.74&0.81&0.84&-&-&-&-\\
&&&&ML&0.59&0.64&0.71&0.81&0.83&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.34}&0.39&\textbf{0.44}&\textbf{0.50}&\textbf{0.51}&-&-&-&-\\
&&&&ML&0.32&0.33&0.40&0.46&\textbf{0.51}&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.31&\textbf{0.40}&0.41&0.49&\textbf{0.51}&-&-&-&-\\
&&&&ML&0.29&0.31&0.39&0.46&0.47&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.62&0.68&0.71&0.72&0.85&0.85&0.87&0.88&0.88\\
&&&&ML&0.58&0.67&0.70&0.71&0.85&0.85&0.87&0.88&0.88\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.35}&0.39&0.41&0.42&\textbf{0.50}&\textbf{0.52}&\textbf{0.55}&\textbf{0.56}&\textbf{0.55}\\
&&&&ML&0.31&0.39&0.39&0.40&\textbf{0.50}&\textbf{0.52}&0.54&0.55&\textbf{0.55}\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&\textbf{0.35}&\textbf{0.43}&\textbf{0.43}&\textbf{0.45}&0.48&\textbf{0.52}&0.52&0.54&\textbf{0.55}\\
&&&&ML&\textbf{0.35}&0.40&0.40&0.42&0.46&0.51&0.51&0.53&\textbf{0.55}\\
\bottomrule
\multirow{12}{*}{et-en}&\multirow{6}{*}{base}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.48&0.51&0.58&0.64&0.67&-&-&-&-\\
&&&&ML&0.42&0.51&0.59&0.67&0.71&-&-&-&-\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.24}&0.26&0.26&0.27&0.29&-&-&-&-\\
&&&&ML&\textbf{0.24}&0.25&0.28&0.29&0.30&-&-&-&-\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.21&\textbf{0.27}&\textbf{0.31}&\textbf{0.31}&\textbf{0.32}&-&-&-&-\\
&&&&ML&0.20&0.21&0.23&0.26&0.29&-&-&-&-\\
\cmidrule{2-14}
&\multirow{6}{*}{large}&\multirow{4}{*}{REG}&\multirow{2}{*}{PC}&BL&0.47&0.54&0.56&0.62&0.69&0.72&0.76&0.77&0.78\\
&&&&ML&0.42&0.54&0.57&0.61&0.72&0.75&0.78&0.80&0.80\\
\cmidrule{5-14}
&&&\multirow{2}{*}{F1}&BL&\textbf{0.25}&0.27&0.24&0.26&0.28&0.28&0.30&0.33&0.31\\
&&&&ML&0.24&0.26&0.25&0.27&0.29&0.30&\textbf{0.32}&0.33&0.33\\
\cmidrule{3-14}
&&\multirow{2}{*}{CLS}&\multirow{2}{*}{F1}&BL&0.24&\textbf{0.31}&\textbf{0.30}&\textbf{0.30}&\textbf{0.31}&\textbf{0.33}&\textbf{0.32}&\textbf{0.35}&\textbf{0.37}\\
&&&&ML&0.21&0.25&0.25&0.25&0.26&0.30&0.31&0.31&0.34\\
\bottomrule
\end{tabular}
\caption{\label{citation-guide}
Mid resource LDs (Micro F1)
}
\end{table*}
